Controlled Experiments on Lane Changing by Transitional Autonomous Vehicle: Dataset and Behavioral Insights

This paper presents the North Carolina Transitional Autonomous Vehicle Lane-Changing (NC-tALC) dataset and uses it to characterize mandatory lane-changing behavior of transitional automated vehicles (tAVs). It quantifies the evolution of lead--lag gaps throughout the lane-change process and examines how potential collision risk develops during the maneuver. A controlled field experiment comprising 78 mandatory lane-change trials was conducted on a public roadway in Apex, North Carolina. Four instrumented vehicles created repeatable traffic conditions while varying the lane changer's initial position within the candidate target gap. High-resolution RTK-GNSS/INS trajectories were processed to identify key timestamps, calculate lead, lag, and lane-change gaps, and estimate interactions using time-gap- and speed-based surrogate safety measures. Despite substantial differences in initial conditions, lead and lag gaps consistently converged toward a relatively narrow range near lane crossing. Potential collision risk increased as the maneuver progressed, peaked near physical lane entry, and was dominated by interactions with the target-lane leader. Lane-change completion did not necessarily coincide with the disappearance of collision risk. This study provides one of the first controlled empirical characterizations of the complete mandatory lane-change process of tAVs using repeatable public-road experiments. The NC-tALC dataset supports analysis of behavioral and safety evolution throughout the maneuver rather than only at the gap-acceptance instant. The dataset and findings provide empirical benchmarks for evaluating automated lane-changing behavior, calibrating behavioral models, and validating simulation and safety assessment methods for mandatory lane-change scenarios.

==> Sections/Experiments_v-1.tex <==
\section{Experiments}
\label{section:Experiments}
This section presents the empirical foundation of the NC-tALC dataset. It is organized into two parts. Subsection~\ref{sec:exp_setup} (\textit{Experiment Setup}) describes the test site and road geometry, the instrumented vehicle platoon, the controlled experimental design and the factors varied across trials, the field-execution protocol, and the trajectory-referencing pipeline. Subsection~\ref{sec:data_examples} (\textit{Examples of Collected Data}) walks through representative trials to illustrate the trajectory-level detail available in the dataset. Behavioral analysis of the collected data is deferred to subsequent studies.

Two complementary experiment series were designed. In the \textbf{Lane-Changing (LC) experiments}, a single tAV executes a mandatory lane change into a platoon of adaptive-cruise-control (ACC)–equipped target vehicles, isolating tAV LC decision and execution behavior. In the \textbf{Responding (Respd) experiments}, two tAVs act as target-lane followers and respond to a cut-in initiated by a third tAV, isolating follower response dynamics. In total, 150 controlled trials were collected (72 LC and 78 Respd), sampled at 20~Hz with centimeter-level RTK-GPS accuracy.

\subsection{Experiment Setup}
\label{sec:exp_setup}

\subsubsection{Test Site and Road Geometry}

The experiments were conducted on a 600~m stretch of Sunset Lake Road in Apex, North Carolina, USA (see Figures~\ref{fig:Test Site} and~\ref{fig:Site Layout}). Sunset Lake Road is a single-lane major collector on which a second lane is intermittently provided to accommodate exclusive right-turn movements. This geometry creates a naturalistic \textit{mandatory} lane-change setting: a vehicle traveling in the exclusive right-turn lane must merge left before the auxiliary lane terminates, so the maneuver is not discretionary.

The selected segment provides two lanes in both the northbound (NB) and southbound (SB) directions, with the rightmost lane in each direction designated exclusively for right turns. The right-turn pavement markings extend approximately 173~m in the NB direction and 169~m in the SB direction, yielding closely comparable layouts; both directions were used for testing. The segment is nearly straight (average heading $331.45\degree$, range $328\degree$–$334\degree$) with negligible grade ($<2\%$); lanes are 3.7~m wide with no shoulder, and no traffic signals are present within the study segment. The posted speed limit is 45~mph. Experiments were carried out over a 10-day period during daylight hours (10:00~AM–5:00~PM) under clear, sunny conditions to ensure consistent visibility. Because the site carries live traffic, all trials were performed without lane closures, preserving realistic ambient-traffic conditions while retaining full control over the four experimental vehicles.

\figTestSite
\SiteLayout

\subsubsection{Vehicles and Instrumentation}

Each trial used a four-vehicle configuration: one lane-changing vehicle, X, plus a three-vehicle target-lane platoon consisting of a lead vehicle, A, a first follower, B, and a second follower, C, as illustrated in Figure~\ref{fig:Vehicle Configuration}. The lead vehicle A was operated in cruise control mode (holding a constant set speed), while X, B, and C were transitional autonomous vehicles (tAVs) with automated lane-change and car-following capabilities. Notably, the same tAV platform served as an ACC target vehicle in the LC experiments and as an autonomously responding follower in the Respd experiments, enabling the two series to be analyzed as a paired initiator–responder corpus.

Every vehicle was instrumented with a high-precision Inertial Navigation System (INS) integrating Real-Time Kinematic (RTK) positioning with a Global Navigation Satellite System (GNSS), an accelerometer, and a gyroscope. The INS provided time-synchronized position, speed, heading, and acceleration at 20~Hz with, per manufacturer specification, centimeter-level positional accuracy and speed accuracy on the order of 0.01~m/s. Each tAV was additionally equipped with in-cabin cameras capturing the forward roadway and dashboard state, and with a CAN interface logging vehicle-reported signals. Device models and accuracy specifications for each vehicle are summarized in Table~\ref{tab:vehicle_instrumentation}.

\figVehicleConfig
\VehicleInstrumentation

\subsubsection{Experimental Design and Scenario Control}

A central objective of the NC-tALC dataset is to deliver \textit{controlled} coverage of the conditions under which a mandatory lane change is initiated; such coverage is difficult to obtain from naturalistic data. Two families of factors were controlled: fixed \textit{driving settings} that define each vehicle's baseline behavior, and \textit{independent variables} that were systematically varied across trials. The driving settings are summarized in Table~\ref{tab:lc_respd_settings}.

\paragraph{Driving settings.}
Each tAV can operate in ACC mode or in fully automated (Auto) mode. In Auto mode, the system exposes an embedded driving-style profile (\textit{Chill}, \textit{Standard}, and \textit{Hurry}) that encodes driving urgency: \textit{Chill} produces relaxed behavior with minimal lane changing, whereas \textit{Hurry} produces more urgent, assertive behavior. Two additional parameters govern the longitudinal profile. \textit{Set speed} is the maximum cruising speed under equilibrium conditions; \textit{speed offset} is the percentage by which a vehicle is permitted to exceed the detected speed limit to match the surrounding flow (e.g., during a lane change). In the LC experiments, the lane-changer X used the \textit{Hurry} setting with a 40\% speed offset (an assertive configuration chosen to reliably elicit active merging), while the ACC followers B and C used a fixed minimum-headway (Headway~2) setting with a 0\% offset, strictly holding the 40~mph set speed.

\paragraph{Independent variables (LC experiments).}
The LC experiments vary the \textit{relative spacing} $s(t) = ds$ and \textit{relative speed} $\Delta v(t) = dv$ of the lane-changer X with respect to the target lead A, both measured at the location $x^*$ and time $t^*$ at which Auto mode is activated (Figure~\ref{fig:Vehicle Configuration}); we refer to this pair jointly as \textit{ds}–\textit{dv}. The activation point $x^*$ was held fixed across trials so that the remaining distance to the lane-drop is not introduced as an uncontrolled third variable and so that no delay is incurred in engaging the lane-change module. The \textit{ds}–\textit{dv} plane was sampled non-uniformly to concentrate trials in conditions expected to challenge automated merging. The sampling is anchored to a nominal 1.5~s target gap discretized into $\sim$5~m (one car-length, $\approx0.3$~s at 40~mph) intervals. Guided by mandatory-LC gap-acceptance behavior in the NGSIM US-101 data, in which human drivers typically accept lead gaps below $\sim$0.6~s and maintain larger following than leading gaps, we distinguish nominally ``easy'' from ``difficult'' merging zones and hypothesize that the difficult zone shifts with $dv$: a favorable speed advantage ($dv>0$) enlarges the easy zone toward larger gaps, whereas a speed deficit ($dv<0$) makes merging near follower B riskier and contracts it. These human-derived boundaries are used only to guide sampling; a tAV may apply different decision rules, so the boundaries are not treated as ground truth for the automated system.

For field execution and sampling, \textit{ds} and \textit{dv} were discretized at $t^*$ into a Discrete Spacing (DS) indicator and a Discrete Velocity (DV) indicator.

The \textbf{Discrete Spacing (DS)} indicator gives the longitudinal position of X relative to the lead A, in four levels:
\begin{itemize}
    \item DS0: X ahead of the lead ($ds<0$);
    \item DS1: parallel to the lead, up to half the target gap ($0<ds<20$~m);
    \item DS2: from half the target gap to follower B ($20<ds<35$~m);
    \item DS3: behind follower B ($ds>35$~m).
\end{itemize}

These four levels define the nominal sampling design. The final DS label of each trial was assigned from its measured longitudinal position at Auto-mode activation rather than from its target bin, so a small number of trials differ from the nominal condition for which they were set up.

The \textbf{Discrete Velocity (DV)} indicator gives the X-to-A speed differential, in three levels:
\begin{itemize}
    \item DV0: speed matched ($\Delta v = 0 \pm 2$~mph);
    \item DV1: X slower ($\Delta v = -5 \pm 2$~mph);
    \item DV2: X faster ($\Delta v = +5 \pm 2$~mph).
\end{itemize}

\paragraph{Independent variables (Respd experiments).}
The Respd experiments isolate how target followers respond to a tAV cut-in. Here B and C operate in Auto mode, and the lane-changer X initiates a cut-in under a fixed near-zero relative speed ($DV=0$, $|dv|<2$~mph) so that spacing remains the primary independent variable. The controlled factor is the \textit{driving-style configuration} of the three tAVs, encoded as a three-letter string [X][B][C] over \textit{Hurry} (H) and \textit{Chill} (C):
\begin{itemize}
    \item \textbf{HHH:} X, B, and C all in \textit{Hurry} mode;
    \item \textbf{HCC:} X in \textit{Hurry}, B and C in \textit{Chill} mode;
    \item \textbf{CHH:} X in \textit{Chill}, B and C in \textit{Hurry} mode;
    \item \textbf{CCC:} X, B, and C all in \textit{Chill} mode.
\end{itemize}
The \textit{Hurry} configuration used a 40\% speed offset and \textit{Chill} a 20\% offset. Spacing conditions followed the same distribution as the LC experiments. These configurations test whether more assertive follower styles (e.g., HHH) yield tighter following or delayed deceleration relative to conservative ones (e.g., HCC, CCC).

\paragraph{Sample distribution.}
The 72 LC trials span nine DS–DV combinations, and the 78 Respd trials span four configurations across three DS levels. The full breakdown is reported in Table~\ref{tab:sample_distribution_combined}, and the joint coverage of the sampled conditions is shown in Figure~\ref{fig:IndependentVariables} for (a) the LC experiments and (b) the Respd experiments.

\ParameterSettings
\SampleSize
\IndependentVariables

\subsubsection{Field Execution Protocol}

To realize each target \textit{ds}–\textit{dv} (or configuration) condition repeatably, a common execution protocol was followed. Prior to entering the two-lane segment, all four vehicles cruised in single-lane formation at a steady 35~mph: the lane-changer X was driven manually at this speed, while the lead A ran in cruise control and followers B and C in ACC or Auto mode with a 40~mph set speed. Upon entering the two-lane stretch, the driver of X manually merged into the exclusive right-turn lane. The lead vehicle A then accelerated from 35 to its 40~mph set speed, followed by B and C, and was required to hold 40~mph steadily for at least 10–15~s before reaching the right-turn markings to establish a consistent target-lane baseline. During this window the driver of X modulated speed and spacing to match the prescribed \textit{ds}–\textit{dv} condition. At the start of the right-turn pavement markings, the driver of X engaged Auto mode; the tAV took over immediately, recognized the exclusive right-turn lane, and executed the mandatory lane change into the left lane. Auto-mode activation therefore constitutes a well-defined handover event $t^*$ and serves as the temporal origin for the controlled initial conditions.

\subsubsection{Trajectory Extraction and Spatial Referencing}

To place all vehicles in a common longitudinal frame, a high-resolution reference map of the site was constructed. A tAV was driven autonomously along each lane in both the NB and SB directions across three trials, logging synchronized INS and video data. The raw GNSS trajectories, recorded in a geographic coordinate system, were converted to a local frame using geodesic distances computed with the WGS-84 model (via Python's \texttt{geopy}). Each lane trajectory was densified to 0.05~m resolution by linear interpolation and resampled at 0.1~m intervals to form smooth left- and right-lane centerlines. The two centerlines were spatially aligned by matching the left-lane point nearest the right-lane start, after which the lateral lane separation was recorded at every 0.1~m station, capturing local road-width variation.

For every trial, the trajectories of all four vehicles were projected onto the left-lane centerline, adopted as the common longitudinal reference axis. At each timestamp the nearest reference station was located, yielding a longitudinal coordinate (position along the lane) and a lateral coordinate (offset from the centerline). To suppress GNSS noise and referencing artifacts, a 20-point ($\approx1$~s) moving average was applied to both position series; speeds were then obtained by differentiating the smoothed longitudinal position and cross-validated against the INS speed channel. This unified spatiotemporal framework enables consistent vehicle-to-vehicle spacing, gap, and relative-speed computation across all trials.

\subsection{Examples of Collected Data}
\label{sec:data_examples}

For each of the 150 trials, the dataset provides fully time-synchronized, 20~Hz trajectories for all four vehicles (A, X, B, C), comprising the raw INS measurements (GNSS position, speed, heading, and acceleration), the map-referenced longitudinal and lateral coordinates on the common left-lane centerline, and derived interaction variables (pairwise spacing, time gap, and relative speed). Each trial is annotated with the Auto-mode activation time $t^*$ and the merge-completion time, together with its experimental metadata (experiment type, DS, DV, driving-style configuration, and travel direction); in-cabin video and CAN logs accompany the tAV records.

To convey the resolution and structure of these trajectories, we walk through two representative trials, one from the LC experiments and one from the Respd experiments. For each, we show both a bird's-eye overlay of vehicle positions on the lane centerlines at key instants and the full set of longitudinal/lateral position, speed, spacing, and time-gap time series. In every time-series panel, the blue vertical line marks Auto-mode activation ($t^*$) and the red vertical line marks merge completion; in the lateral-position panels, the zero line is the left-lane centerline and the $\approx$3.7~m level is the right-lane centerline.

\paragraph{LC Example: decelerate-then-merge ($DS=1$, $DV=0$).}
Figure~\ref{fig:OverlayTrajectories} overlays vehicle positions at $t=24$, 31, and 35~s for a trial in which X starts parallel to the lead A ($DS=1$) with matched speed ($DV=0$); Figure~\ref{fig:Sample Example LC Experiments} gives the corresponding trajectories. At $t=24$~s X reaches the right-turn markings and the driver engages Auto mode; the tAV immediately signals intent (left blinker), decelerates, and remains in the subject lane for a further 4–5~s of longitudinal adjustment. Because its speed is slightly below A's, the lead spacing grows during this interval. Lateral motion begins near $t=29$~s and the merge completes by $t\approx34$~s, with a residual speed difference of $\approx$0.4~m/s relative to A. The maneuver reduces follower B's speed by $\approx$1.5~m/s. Such execution, in which the tAV's longitudinal strategy directly shapes the follower's response, is precisely the interaction the NC-tALC dataset is designed to expose.

\OverlayTrajectories

\paragraph{Respd Example: follower response to a cut-in ($DS=0$, HHH).}
Figure~\ref{fig:Sample Example Respd Experiments} shows a Respd trial with $ds=0$~m under the HHH configuration, in which the lane-changer X and both followers operate in \textit{Hurry} mode. Prior to activation, the autonomous followers exhibit greater speed variability than the lead A, reflecting their higher set speed plus offset, while A (cruise control) holds a steady 40~mph reference. X engages Auto mode at $t=22$~s and begins decelerating within 1~s to adjust its longitudinal profile; at $t\approx28$~s it initiates the lateral maneuver at reduced speed, carrying a $\approx$1.8~m/s relative speed, and completes the lane change with a residual $\approx$1~m/s difference after speed-matching. The synchronized follower trajectories capture the induced response in full, supporting analysis of response timing and intensity as a function of driving style, the central question of the Respd series.

\SampleExampleCombined

==> Sections/Introduction_v-1.tex <==
\section{Introduction}

Vehicles operating beyond conventional SAE Level 1--2 automation but short of full autonomy---referred to in this study as transitional autonomous vehicles (tAVs)---are increasingly present on public roadways \cite{Ammourah2024IntroductionExtraction}. What distinguishes tAVs from the Level 1--2 systems that preceded them is not incremental improvement in longitudinal control but the addition of a qualitatively new capability: automated lane changing. Whereas adaptive cruise control (ACC) and lane-keeping assist regulate motion within a lane, a tAV can select a gap in an adjacent lane, commit to it, and execute the maneuver autonomously under driver supervision. Lane changing thus moves from a task the driver performs to a task the vehicle performs, and a maneuver that is already among the most safety-critical in everyday driving---accounting for roughly 4.2\% of police-reported crashes in the United States \cite{NHTSA2022SummarySystems}---is now executed by a controller whose behavior has not been characterized. Beyond crash risk, lane changing requires tactical decisions such as gap selection under time pressure, and its effects extend to traffic capacity as well as safety, contributing to disturbances and bottlenecks even absent a collision \cite{Cassidy1999SomeBottlenecks, Shi2021EmpiricalSettings, Zheng2014RecentChanging}.

There is little basis for assuming that tAV lateral behavior resembles that of human-driven vehicles (HDVs) or Level 4 automated vehicles. Little is known about the lane-change decision logic and execution algorithms implemented in commercial tAVs because these systems are proprietary. At the same time, there is no evidence that tAV behavior resembles that of Level 4 automated vehicles, as tAVs operate under driver supervision and may be designed to satisfy different regulatory and functional requirements. Their lateral behavior is therefore likely to occupy a distinct regime, with consequences for the gaps they accept, the disturbances they impose on surrounding traffic, and the resulting effects on traffic flow and safety. Empirical studies of this behavior, however, are almost entirely absent.

 The availability of automated vehicle trajectories from the Waymo Open Motion Dataset (WOMD) \cite{Hu2023AutonomousModelling} has enabled researchers to explore behavioral differences between automated and human-driven vehicles. Analyses of these data have established that Level 4 AVs adopt larger lead and lag gaps, longer execution times, and lower acceleration variability than human drivers \cite{Ali2024InvestigatingDataset}, that following vehicles exhibit lower volatility and reduced crash risk \cite{Wen2023AnalysisData}, and yet that AV-initiated lane changes can provoke abrupt human responses and elevate rear-end risk \cite{Ali2025AutonomousFollower}. Controlled experimental campaigns, in contrast, have concentrated on Level 1 longitudinal behavior---OpenACC \cite{Makridis2021OpenACC.Systems}, the Vanderbilt ACC experiments \cite{Gunter2021AreStable}, and the MA ACC campaign \cite{Li2021Car-followingExperiments}---establishing car-following and string-stability properties of commercial ACC systems, but by construction saying nothing about lateral maneuvers.

Data on tAVs specifically remain limited to two sources, neither of which provides a comprehensive characterization of tAV lane-changing behavior. The Third Generation Simulation (TGSIM) dataset \cite{Ammourah2024IntroductionExtraction} captures Level 1--3 automated vehicles in naturalistic highway and urban environments using aerial and infrastructure-based videography. Although the dataset includes mandatory lane-change scenarios, its Level 2 subset contains only a limited number of lane-change cases, and published studies have not yet provided an empirical characterization of tAV lane-changing behavior. Existing analyses have instead focused on discretionary lane changes while pooling Level 1 and Level 2 vehicles, rather than isolating mandatory lane-changing behavior of tAVs \cite{Zhang2025InvestigationDataset}. The JRC campaign of \cite{Mattas2025SafetyExperiments} comes closest to the present work: five ADAS-equipped vehicles with assisted lane-change functionality were driven on I-24 near Nashville, TN, and a range of assisted lane-change modes, including driver-requested, driver-confirmed, system-initiated, and interrupted maneuvers, were evaluated in live traffic. The study found that each system exhibited consistent lane-change behavior, with four of five executing lane changes at lower speeds and decelerations than human drivers while one completed the maneuver assertively in roughly five seconds; safety margins could be evaluated for only three vehicles, and their designs were found not to conform to the critical-distance requirements of UN Regulations 79 and 171. That campaign, however, examines discretionary assisted lane changes with only the ego vehicle instrumented and surrounding traffic uncontrolled, so the conditions under which each maneuver is initiated are observed rather than prescribed, and the responses of surrounding vehicles are not measured. Furthermore, the data are not publicly available.

Two gaps follow. First, no controlled experiment on tAV exists: the surrounding vehicles have never been instrumented and the initial conditions of a tAV lane change---relative speed, spacing, and follower mode---have never been systematically varied, so tAV behavior cannot be attributed to the conditions that produce it. Second, and consequently, there is limited empirical characterization of tAV lateral behavior, leaving the effects of tAVs on traffic flow and safety unknown at precisely the maneuver where those effects are most likely to arise.

To address these gaps, this study presents a controlled experimental campaign in which a tAV perform mandatory lane changes on an exclusive right-turn lane under repeatable and systematically varied conditions, with all vehicle trajectories recorded using high-precision RTK-GPS instrumentation. The resulting dataset is referred to as the North Carolina Transitional Autonomous Vehicle Lane-Changing (NC-tALC) Dataset: 150 trials across two configurations. In the LC experiments, a tAV changes lanes into a target lane occupied by ACC-equipped vehicles across selectively varied relative speed and spacing. In the responding (Respd) experiments, two tAVs act as followers to a cut-in performed by another tAV, with variation in driving mode and lane-changer relative spacing. Unlike large naturalistic datasets, NC-tALC provides repeatable mandatory lane-change scenarios and paired follower response trajectories, enabling controlled cause-and-effect analyses that are seldom achievable under naturalistic driving conditions. Using this dataset, we characterize tAV driving behavior throughout the lane-change process. Using data from the Respd experiments, two findings are central: (a) The lead--lag gap distribution converges to a narrow region at lane crossing despite varying initial conditions, and (b) substantial collision risk develops during tAV lane changes, predominantly with the target-lane leader, peaking at lane entry and persisting beyond the lane-change end.

The remainder of the paper is organized as follows. Section~\ref{section:Experiments} describes the experimental design, Section~\ref{section:Methods and Materials} describes methods and materials, Section~\ref{sec:gap-evolution} and Section ~\ref{section:Risk Assessment} describe the finding on gap-evolution and risk assessment and Section~\ref{sec:conclusion} presents conclusions and implications.





==> Sections/Methods.tex <==
\section{Methods and Materials}
\label{section:Methods and Materials}
\subsection{Data and Trajectory Processing}

Each vehicle is instrumented with a single INS unit integrating RTK-GNSS positioning, an accelerometer, and a gyroscope, mounted at the vehicle center. The INS provides time-synchronized position, speed, heading, and acceleration at 20~Hz, with centimeter-level positional accuracy and speed accuracy on the order of 0.01~m/s. Vehicle speed is taken from the INS velocity channel.

The raw GNSS trajectories are converted to a local coordinate frame using geodesic distances under the WGS-84 model through Python's \texttt{geopy} library and projected onto the left-lane centerline as the common longitudinal reference axis. This process yields a longitudinal coordinate, representing position along the lane, and a lateral coordinate, representing the offset from the centerline, for each vehicle at each timestamp. The resulting trajectories represent the vehicle center.

To suppress GNSS noise and referencing artifacts, a 20-point moving average, corresponding to approximately 1~s, is applied to both the longitudinal and lateral position series to produce the trajectories used for analysis. Speed is then obtained by differentiating the smoothed longitudinal position and is cross-validated against the INS speed channel.

\subsection{Road and Lane Geometry}

To place all vehicles in a common longitudinal frame, a high-resolution reference map of each study site is constructed. A tAV was driven in autonomous mode along each lane in both the northbound and southbound directions, and its position, representing the vehicle center, was used to approximate the lane centerline. The autonomous controller was expected to maintain the vehicle near the lane center more consistently than a human driver, thereby providing a more consistent reference trajectory.

Three repetitions were completed for each lane to reduce trajectory fluctuations and improve mapping accuracy. The resulting trajectories were first densified to a resolution of 0.05~m using linear interpolation and then resampled at 0.1~m intervals to form smooth left- and right-lane centerlines. The centerlines were spatially aligned by matching the point on the left-lane centerline nearest to the starting point of the right-lane centerline.

The lateral separation between the lane centerlines was recorded at every 0.1~m station to capture local variations in road geometry. The lane widths were 3.7~m at Site~1 and 4.0~m at Site~2.
\subsection{Key Timestamps}

Each trial is annotated with nine key timestamps that mark the progression of the lane-change maneuver: Auto-mode Activation (ACT), LC Start (LCS), Left Edge Touching (LET), LC Crossing (LCC), LC End (LCE), and four post-LCE offsets at +2.5, +5, +7.5, and +10~s. All variables analyzed in the subsequent sections are sampled at these timestamps.

ACT ($t^{*}$) marks the moment the driver engages Auto mode at the start of the right-turn pavement markings, after which the tAV immediately assumes control. It is annotated from the synchronized video records. ACT represents the first instant of full tAV authority, at which the human driver monitors but no longer maneuvers, and defines the controlled initial conditions ($d_s$, $d_v$).

LCS marks the onset of the lane-change maneuver and is identified by tracking the lateral movement of the vehicle center. Starting from LCC, the trajectory is searched backward until the smoothed lateral velocity first exceeds a threshold of 0.05~m/s toward the target lane, defining the start of continuous lateral motion.

LET is the moment the left edge of the lane-changing tAV reaches the target-lane boundary, representing the first instant that the vehicle physically enters the target lane. It is identified by first determining the vehicle-center position at LCC, computing the lateral offset from the vehicle center to the left-front corner using the vehicle geometry and heading angle, and then linearly interpolating the lateral trajectory to determine the instant when the left-front corner reaches the lane boundary.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\textwidth]{Figures/LET_LCC.png}
    \caption{Illustration of LET (Left Edge Touching) and LCC (Lane Crossing) used for event identification.}
    \label{fig:LET_LCC}
\end{figure}

LCC is the moment the center of the lane-changing vehicle crosses the lane boundary and is identified by linearly interpolating the vehicle-center trajectory to the point where the vehicle center is equidistant from the mapped left- and right-lane centerlines.

LCE marks the completion of the lane-change maneuver, indicating that the lane-changing vehicle has fully entered the target lane and stabilized its lateral position. Starting from LCC, the trajectory is searched forward until the smoothed lateral velocity falls below 0.05~m/s and remains below this threshold for at least 0.3~s while the vehicle center remains within the target lane.

The four post-LCE offsets (+2.5, +5, +7.5, and +10~s) are fixed time intervals referenced from LCE and are used to examine the post-maneuver evolution of the variables of interest.
